LQER: Low-Rank Quantization Error Reconstruction for LLMs

Post-training quantization of Large Language Models (LLMs) is challenging. In this work, we introduce Low-rank Quantization Error Reduction (LQER), which combines quantization and low-rank approximation to recover the model capability. LQER leverages an activation-induced scale matrix to drive the singular value distribution of quantization error towards a desirable distribution, which enables nearly-lossless W4A8 quantization on various LLMs and downstream tasks without the need for knowledge distillation, grid search, or gradient-base iterative optimization. Unlike existing methods, the computation pattern of LQER eliminates the need for specialized Scatter and Gather processes to collect high-precision weights from irregular memory locations. Our W4A8 LLMs achieve near-lossless performance on six popular downstream tasks, while using 1.36$\times$ fewer hardware resources than the leading state-of-the-art method. We open-source our framework at https://github.com/ChengZhang-98/lqer

==> figures/placeholders/s4-ablation-study-dsvd-vs-from-scratch.tex <==
\begin{figure}
    \vskip 0.2in
    \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/placeholders/s4-ablation-study-dsvd-vs-from-scratch.png}
    \caption{Learned singular value distribution vs initialization methods. \LRQd{} initializes $S$ using activation-induced $S$ like \LRQa{}. We also tried initializing $S$ using identity matrix such that the optimization starts from \LRQa{}, and train it from scratch. We observe that the identity-initialized $S$ fails to converge to a distribution better than the activation-induced $S$. This shows that the activation-induced $S$ is an effective initialization for \LRQd{}, and training $S$ from scratch is challenging.}
    \label{fig:s4:ablation-study-dsvd-vs-from-scratch}
    \end{center}
    \vskip -0.2in
\end{figure}

==> figures/s1-llm-int8-vs-lqer.tex <==
\begin{figure*}
    \vskip 0.2in
    \begin{center}
        \includegraphics[width=0.6\textwidth]{figures/img_src/s1-llm-int8-vs-lqer.pdf}
        \caption{Comparison of QLoRA, \texttt{LLM.int8()}, and \LRQ{}. QLoRA (left) is a parameter-efficient fine-tuning method that updates two low-rank BF16 matrices, $L_1$ and $L_2$, using gradient descent in the training stage, and fuse them back to a single BF16 matrix, $W'=W+L_1L_2$, before the inference stage. $Q^{-1}(\cdot)$ denotes double-dequantization from 4-bit NormalFloat\cz{cite me} to BF16 in QLoRA. \texttt{LLM.int8()} decompose one FP16 matrix multiply ($XW$) into a FP16 sub-matrix multiply ($X_1W_1$) and a 8-bit fixed-point multiply ($X_{2,q}W_{2,q}$) using an activation threshold $\tau$ at runtime. \texttt{LLM.int8()} requires extra cost of threshold, gather, and scatter. Our method is a PTQ method that does not target fine-tuning. Instead, we use SVD to create two deterministic small high-precision matrices, $A_k$, and $B_k$, to compensate the quantization error of aggressive weight quantization. In the reference stage, \LRQ{} runs one low-precision but large matrix multiply ($XW_q$) and two high-precision but small matrix multiplies ($XA_k$ and $(XA_k)B_k$) in parallel to improve hardware efficiency.}
        \label{fig:s4:qlora-vs-llm-int8-vs-lrhp}
    \end{center}
    \vskip -0.2in
\end{figure*}

==> figures/s1-motivation.tex <==
\begin{figure}[t]
    %\vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=0.5\textwidth]{figures/img_src/Q-error-comparison.pdf}}
        \vskip -0.1in
        \caption{We apply SVD to the quantization error $E_q=W-W_q$ (scaled one for \LRQa{}) for a 3-bit fixed-point quantized weight in OPT-1.3B, and plot their singular values. All singular values are normalized for a fair comparison\textsuperscript{\ref{footnote:normalization-in-fig1}}. Curves with a more skewed trend suggest higher suitability for low-rank approximation. Our \LRQa{} displays a much steeper distribution with a smaller number of dominating singular values. \cz{help needed.}}
        \label{fig:s1:q-error-comparison}
    \end{center}
    \vskip -0.2in
\end{figure}


